Multidimensional Contours \`a la Fr\"{o}hlich-Spencer and Boundary Conditions for Quantum Spin Systems

In this thesis, we present results from the investigation of two problems, one related to the phase transition of long-range Ising models and the other one associated with the characterization of equilibrium states in quantum spin systems. Due to the long-range nature of the interactions, $J|x-y|^{-\alpha}$, estimates using contours usually found in the literature have restrictions on the range of interactions ($\alpha>d+1$ in Ginibre, Grossmann, and Ruelle in 1966 and Park in 1988 for discrete spin systems and possibly non-symmetric situations but with the restrictions $\alpha>3d+1 $). We were able to extend the phase transition argument for long-range Ising-type models to the entire region $\alpha>d$ using the multi-scale arguments presented in the articles by Fr\"ohlich and Spencer. In quantum statistical mechanics, the KMS condition is used as a characterization for the equilibrium states of the system. Widely studied today, it is known to be equivalent to other equilibrium notions such as the variational principle. We present another possible characterization of equilibrium states in quantum spin systems by generalizing the DLR equations to the quantum context using Poisson point process representations. We also discuss the relationship of these quantum DLR equations with the KMS states of a subclass of interactions that contains the Ising model with a transverse field.

==> Figuras/caixas_loucas.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,338); %set diagram left start at 0, and has height of 338

%Shape: L Shape [id:dp31493122358252] 
\draw  [line width=2.25]  (120.65,130.65) -- (120.48,187.01) -- (81.84,186.9) -- (81.72,228.53) -- (19.35,228.35) -- (19.65,130.35) -- cycle ;
%Shape: L Shape [id:dp5690399127255712] 
\draw  [line width=2.25]  (296.65,231.65) -- (296.48,288.01) -- (257.84,287.9) -- (257.72,329.53) -- (195.35,329.35) -- (195.65,231.35) -- cycle ;
%Shape: L Shape [id:dp2982836578210307] 
\draw  [line width=2.25]  (296.65,18.65) -- (296.48,75.01) -- (257.84,74.9) -- (257.72,116.53) -- (195.35,116.35) -- (195.65,18.35) -- cycle ;
%Shape: L Shape [id:dp8730707897090977] 
\draw  [line width=2.25]  (469.65,120.65) -- (469.48,177.01) -- (430.84,176.9) -- (430.72,218.53) -- (368.35,218.35) -- (368.65,120.35) -- cycle ;
%Shape: Square [id:dp3156013900408027] 
\draw  [color={rgb, 255:red, 13; green, 25; blue, 231 }  ,draw opacity=1 ][line width=2.25]  (426.5,134.5) -- (454.5,134.5) -- (454.5,162.5) -- (426.5,162.5) -- cycle ;
%Shape: Square [id:dp7060674423693782] 
\draw  [color={rgb, 255:red, 13; green, 25; blue, 231 }  ,draw opacity=1 ][line width=2.25]  (385,178) -- (413.5,178) -- (413.5,206.5) -- (385,206.5) -- cycle ;

%Shape: L Shape [id:dp6757269670016743] 
\draw  [color={rgb, 255:red, 13; green, 25; blue, 231 }  ,draw opacity=1 ][line width=2.25]  (281.62,33.99) -- (281.54,58.2) -- (239.15,58.07) -- (239.02,100.97) -- (214.52,100.9) -- (214.71,33.8) -- cycle ;
%Shape: Square [id:dp4714323543505231] 
\draw  [color={rgb, 255:red, 13; green, 25; blue, 231 }  ,draw opacity=1 ][line width=2.25]  (213,289) -- (241.5,289) -- (241.5,317.5) -- (213,317.5) -- cycle ;
%Curve Lines [id:da25521161032643525] 
\draw [line width=2.25]    (68.5,120) .. controls (83.05,67.62) and (127.71,55.7) .. (180.57,53.21) ;
\draw [shift={(185.5,53)}, rotate = 177.92] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;
%Shape: Boxed Bezier Curve [id:dp4487089839352797] 
\draw [line width=2.25]    (64.5,238) .. controls (79.05,290.38) and (123.71,302.3) .. (176.57,304.79) ;
\draw [shift={(181.5,305)}, rotate = 182.08] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;
%Curve Lines [id:da8844155020445116] 
\draw [line width=2.25]    (422.81,104.49) .. controls (406.2,55.24) and (360.58,44.93) .. (307.5,43) ;
\draw [shift={(424.5,110)}, rotate = 254.48] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;
%Shape: Boxed Bezier Curve [id:dp243847581038675] 
\draw [line width=2.25]    (420.81,237.51) .. controls (404.2,286.76) and (358.58,297.07) .. (305.5,299) ;
\draw [shift={(422.5,232)}, rotate = 105.52] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (16.07,-7.72) -- (0,0) -- (16.07,7.72) -- (10.67,0) -- cycle    ;

% Text Node
\draw (78,27) node [anchor=north west][inner sep=0.75pt]  [font=\LARGE] [align=left] {$\displaystyle B_{1}$};
% Text Node
\draw (396,28) node [anchor=north west][inner sep=0.75pt]  [font=\LARGE] [align=left] {$\displaystyle B_{2}$};
% Text Node
\draw (80,296) node [anchor=north west][inner sep=0.75pt]  [font=\LARGE] [align=left] {$\displaystyle B_{1} '$};
% Text Node
\draw (380,288) node [anchor=north west][inner sep=0.75pt]  [font=\LARGE] [align=left] {$\displaystyle B_{2} '$};


\end{tikzpicture}


==> Makefile <==
# 
# makefile para a compilação do documento
#
# Sáb Jun 23 21:13:37 BRT 2007
#

BASE_NAME = tese-exemplo

LATEX     = latex
PDFLATEX  = pdflatex
BIBTEX    = bibtex
MAKEINDEX = makeindex

pdf: $(BASE_NAME).pdf
ps: $(BASE_NAME).ps

$(BASE_NAME).pdf: $(BASE_NAME).tex 
	$(PDFLATEX) $<
	$(BIBTEX) $(BASE_NAME) 
	$(MAKEINDEX) $(BASE_NAME) 
	$(PDFLATEX) $< 
	$(PDFLATEX) $<
	$(PDFLATEX) $<

$(BASE_NAME).ps: $(BASE_NAME).tex 
	$(LATEX) $<
	$(BIBTEX) $(BASE_NAME) 
	$(MAKEINDEX) $(BASE_NAME) 
	$(LATEX) $< 
	$(LATEX) $<
	$(LATEX) $<
	
clean:
	rm -f $(BASE_NAME)*.ps $(BASE_NAME)*.dvi *.log \
	      *.aux *.blg *.toc *.brf *.ilg *.ind \
	      missfont.log $(BASE_NAME)*.bbl $(BASE_NAME)*.pdf $(BASE_NAME)*.out \
		  $(BASE_NAME)*.lof $(BASE_NAME)*.lot 

